Consistent Query Answering under Spatial Semantic Constraints

Consistent query answering is an inconsistency tolerant approach to obtaining semantically correct answers from a database that may be inconsistent with respect to its integrity constraints. In this work we formalize the notion of consistent query answer for spatial databases and spatial semantic integrity constraints. In order to do this, we first characterize conflicting spatial data, and next, we define admissible instances that restore consistency while staying close to the original instance. In this way we obtain a repair semantics, which is used as an instrumental concept to define and possibly derive consistent query answers. We then concentrate on a class of spatial denial constraints and spatial queries for which there exists an efficient strategy to compute consistent query answers. This study applies inconsistency tolerance in spatial databases, rising research issues that shift the goal from the consistency of a spatial database to the consistency of query answering.

==> macros.tex <==
\usepackage{color}
\usepackage{amssymb,xspace,latexsym,epic,eepic,graphicx}
\usepackage{epsfig,amsmath}
\usepackage{hhline}
\usepackage{times}
\usepackage[lflt]{floatflt}
\usepackage{multicol}
\usepackage[lflt]{floatflt}
\usepackage{multicol}
\usepackage{setspace}

\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newcommand{\defproofN}[2]{{\vspace{0.3 cm} \noindent\it Proof of
#1:\ }#2}

\newcommand{\hproof}[1]{{\noindent\bf Proof:~~ }#1 \boxtheorem
\newline \newline
\noindent} % here proof
\newcommand {\rpr}[2]{{\it Repairs\/}_{#1}({#2})}
\newcommand{\boxtheorem}{\hfill $\Box$}
\newcommand{\ignore}[1]{}
\newcommand{\nit}[1]{{\it #1}}
\newcommand{\n}{~{\it not}~}
\newcommand{\MC}{\nit{MPC}}
\newcommand{\go}{g_\oslash}
\newcommand{\D}{\nit{D}}
\newcommand{\SD}{\nit{D}}

\newcommand{\defproof}[2]{{\noindent\bf Proof:\
}#2}

\newcommand{\red}[1]{{\em \bf\textcolor[rgb]{1.00,0.00,0.00}{[#1]}}}
\newcommand {\blue}[1]{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
\newcommand {\green}[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}

\newcommand{\commonica}[1]{{\vspace{2mm}\noindent \bf \green{COMMONICA:}}~ #1 \hfill \green{\bf {END.}}\\}
\newcommand{\comlb}[1]{{\vspace{2mm}\noindent \bf \red{COMM(LEO):}}~ #1 \hfill \red{\bf {END.}\vspace{3mm}}\\ }
\newcommand{\comandrea}[1]{{\vspace{2mm}\noindent \bf \blue{COMANDREA:}}~ #1 \hfill \blue{\bf {END.}}\\}
\newcommand{\comchicas}[1]{{\vspace{2mm}\noindent \bf \green{COMENTARIO:}}~ #1 \hfill \green{\bf {END.}}\\}

